V2V4Real: A Real-world Large-scale Dataset for Vehicle-to-Vehicle Cooperative Perception

Modern perception systems of autonomous vehicles are known to be sensitive to occlusions and lack the capability of long perceiving range. It has been one of the key bottlenecks that prevents Level 5 autonomy. Recent research has demonstrated that the Vehicle-to-Vehicle (V2V) cooperative perception system has great potential to revolutionize the autonomous driving industry. However, the lack of a real-world dataset hinders the progress of this field. To facilitate the development of cooperative perception, we present V2V4Real, the first large-scale real-world multi-modal dataset for V2V perception. The data is collected by two vehicles equipped with multi-modal sensors driving together through diverse scenarios. Our V2V4Real dataset covers a driving area of 410 km, comprising 20K LiDAR frames, 40K RGB frames, 240K annotated 3D bounding boxes for 5 classes, and HDMaps that cover all the driving routes. V2V4Real introduces three perception tasks, including cooperative 3D object detection, cooperative 3D object tracking, and Sim2Real domain adaptation for cooperative perception. We provide comprehensive benchmarks of recent cooperative perception algorithms on three tasks. The V2V4Real dataset can be found at https://research.seas.ucla.edu/mobility-lab/v2v4real/.

==> tables/da_old.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|l|c}
\hline
Method   & Domain Adaptation      & \multicolumn{1}{l}{AP@IoU=0.5} \\ \hline
AttFuse  & \multicolumn{1}{c|}{x} & 15.2~($\downarrow$ 32.7)                            \\
AttFuse  & \multicolumn{1}{c|}{\checkmark}                        & 21.4~($\downarrow$ 26.5)                           \\
F-Cooper & \multicolumn{1}{c|}{x} & 19.9~($\downarrow$ 25.7)                           \\
F-Cooper & \multicolumn{1}{c|}{\checkmark}                         & 26.4~($\downarrow$ 19.2)             \\
V2VNet   & \multicolumn{1}{c|}{x} & 14.7~($\downarrow$ 27.3)                           \\
V2VNet   &  \multicolumn{1}{c|}{\checkmark}                       & 19.7~($\downarrow$ 22.3)          \\
V2X-ViT  &  \multicolumn{1}{c|}{x}                       & 23.7~($\downarrow$ 25.2)          \\
V2X-ViT  & \multicolumn{1}{c|}{\checkmark}                        & 29.0~($\downarrow$ 19.9)         \\
CoBEVT   & \multicolumn{1}{c|}{x} & 22.3~($\downarrow$ 28.8)                           \\
CoBEVT   &  \multicolumn{1}{c|}{\checkmark}                       & 27.1~(($\downarrow$ 24)                              \\ \hline
\end{tabular}
\caption{Domain Adaptation benchmark. The number in the bracket indicates the precision drop compared to training on the V2V4Real dataset.}
\label{tab:da_old}
\end{table}
